Foraging with MUSHROOMS: A Mixed-Integer Linear Programming Scheduler for Multimessenger Target of Opportunity Searches with the Zwicky Transient Facility

Electromagnetic follow-up of gravitational wave detections is very resource intensive, taking up hours of limited observation time on dozens of telescopes. Creating more efficient schedules for follow-up will lead to a commensurate increase in counterpart location efficiency without using more telescope time. Widely used in operations research and telescope scheduling, mixed integer linear programming (MILP) is a strong candidate to produce these higher-efficiency schedules, as it can make use of powerful commercial solvers that find globally optimal solutions to provided problems . We detail a new target of opportunity scheduling algorithm designed with Zwicky Transient Facility in mind that uses mixed integer linear programming. We compare its performance to \texttt{gwemopt}, the tuned heuristic scheduler used by the Zwicky Transient Facility and other facilities during the third LIGO-Virgo gravitational wave observing run. This new algorithm uses variable-length observing blocks to enforce cadence requirements and ensure field observability, along with having a secondary optimization step to minimize slew time. \blue{We show that by employing a hybrid method utilizing both this scheduler and \texttt{gwemopt}, the previous scheduler used, in concert, we can achieve an average improvement in detection efficiency of 3\%-11\% over \texttt{gwemopt} alone} for a simulated binary neutron star merger data set consistent with LIGO-Virgo's third observing run, highlighting the potential of mixed integer target of opportunity schedulers for future multimessenger follow-up surveys.

==> uvex.tex <==
\iffalse
%This is the old abstract
Here, we detail the software and diagnostic studies related to the UVEX survey cadence studies.
We rely on Integer Linear Programming to optimize an observing plan 1/4 orbit at a time, which allows us to easily control the percentage of the baseline survey vs. boutique surveys.
This analysis does not (yet) minimize slew times between each observation.
Our optimization metric is the volumetric rate of sky covered constrained on parameters like time since last observation.

\appendix
\section{Stuff that was here before B started writing}
Notes on how to think about this process are as follows:
\begin{enumerate}
    \item Ask science questions: how does the cadence improve our ability to measure RR Lyrae periods? how does the cadence affect our ability to measure colors of TDEs?
    \item Propose a cadence to maximize the difference between objects (in a $k$-means sense): can we separate TDEs from UV-flares in an AGN?
    \item Get to the science as fast as possible: should cover the whole sky once early for MMA sources and then back off to work on the surveys
    \item Science groups: should derive simulated characteristics of observables (i.e. the rise time of a TDE flare)
\end{enumerate}

Our paper is structured as follows. We start by describing UVEX and requirements for its scheduler in Section~\ref{sec:requirements}. We then describe the scheduling of these observations and their coverage of multi-messenger events in Section~\ref{sec:observing}. We then discuss the efficiency of counterpart detection for each of these strategies in Section~\ref{sec:results}, and summarize our conclusions and future outlook in Section~\ref{sec:summary}.


\section{UVEX Requirements}
\label{sec:requirements}

The UVEX baseline survey ($\sim$\,50\% of the time) seeks to cover the entire sky for $\sim$\,10\,ks in each field.
One of the main goals for this work is to determine the cadence and exposure times used to reach this requirement.
In addition, there will be boutique surveys that seek to address specific science goals, which must run in coordination with the baseline survey.
Those surveys simulated so far cover:

\begin{itemize}
    \item Baseline survey ($\sim$\,50\% of the time): cover the entire sky for $\sim$\,10\,ks in each field.
    \item ``Kilonovae'' ($\sim$\,20\% of the time): cover $\sim 225$\,sq. deg. repeatedly to search for fast transients
    \item ``Galactic Plane'' ($\sim$\,20\% of the time): cover the Galactic Plane repeatedly to have sufficient epochs for period searches
    \item ``GWs'' ($\sim$\,10\% of the time): cover GW candidate skymaps
\end{itemize}

Thus, the UVEX scheduler should
\begin{itemize}
    \item Select pointings from a fixed field grid (assumes square fields 3.3$^\circ$ on a side.
    \item Conduct the surveys described previously, balancing observing time between programs that take advantage of observations within the baseline program
    \item Maximize an observing efficiency metric and prioritize cadence control.
\end{itemize}

\section{Observing Programs}
\label{sec:observing}

\begin{figure*}
\begin{center}
 \includegraphics[width=3.5in]{figures/counts_all_FUV.png}
 \includegraphics[width=3.5in]{figures/counts_baseline_FUV.png}
 \includegraphics[width=3.5in]{figures/counts_GW_FUV.png}
 \includegraphics[width=3.5in]{figures/counts_kilonova_FUV.png}
  \caption{Optimized schedule for an example UVEX survey with 2D skymaps with tiles covered by the example observations. The top left panel shows observations from all surveys, the top right the baseline survey, the bottom left the gravitational waves, and the bottom right the time domain field.}
 \label{fig:survey}
\end{center}
\end{figure*}

We aim to determine a survey strategy for UVEX consistent with the goals described above.
To do so, we begin with the MIP-based scheduler developed for Dorado\footnote{https://github.com/nasa/dorado-scheduling}. 
This scheduler relies on the Healpix-basis \cite{GoHi2005} to perform gravitational-wave follow-up.
We extend this infrastructure to use ``skymaps'' developed for each particular science case.
For example, the baseline skymap is a normalized probability distribution where pixels yet to be observed are set to 1 and pixels already observed are set to 0.01; the skymap used in the kilonova and galactic plane distribution is the same, except only in the fields selected for those observations. The gravitational-wave follow-up is drawn from examples of O5-era skymaps.

The scheduler attempts to maximize probability in each skymap subject to the constraints imposed by program balance and cadence.
Each program is defined by a number of quantities:

\begin{enumerate}
\item footprint on the sky (a discrete set of fields, which may be larger than the set observable in one observing block)
\item the fraction of the telescope observing time they are allocated
\item the number of nights between successive revisits to this field for this program (with knowledge of the other programs) (i.e., the ``inter-night gap,'' such as a 1-day or 3-day cadence);
\item the number of visits and filter set for observations requested within a night (e.g., two nightly visits, one in $NUV$-band and one in $FUV$-band).
\end{enumerate}

For each quarter orbit, we draw a program consistent with its probability of being executed, and create the corresponding skymap.
The scheduling algorithm then determines which fields are observed at which times.
We have implemented the scheduling algorithm as a Python library, which is publicly available\footnote{\url{https://github.com/nasa/dorado-scheduling}} under an open source license.
The scheduler code takes advantage of a range of open-source Python libraries, including \texttt{Astropy} \citep{PrSi2018} and \texttt{Astroplan} \citep{MoTo2018}.
We use the commercial optimization package CPLEX\footnote{https://www.ibm.com/analytics/cplex-optimizer} under an academic license to perform the core ILP optimization.

\rednote{WE NEED TO KEEP OBSERVING CONSTRAINTS WHEN DOING THIS!}.
We use a second optimization process to sequence observations efficiently within each block.
We compute the pairwise slew times between all fields assigned to a block, and then solve the Traveling Salesman Problem (TSP)
as an ILP problem in CPLEX.
In our application the quantity to be minimized is not the total length of the salesman's tour, but the total time spent slewing between fields within the block.

\subsection{Parameters}

\begin{align}
N_\mathrm{grid} &\quad\textrm{number of fields in grid} \\
N_\mathrm{field} &\quad\textrm{number of fields selected} \\
N_\mathrm{visit} &\quad\textrm{number of visits} \\
N_\mathrm{pix} &\quad\textrm{number of HEALPix pixels} \\
\left\{U_l\right\}_{l=1}^{N_\mathrm{pix}} &\quad\textrm{set of fields that contain pixel }l \\
E &\quad\textrm{exposure time} \\
\left\{S_i, T_i\right\}_{i=1}^{N_\mathrm{grid}} &\quad\textrm{rise and set times of field }i \\
\left\{P_l\right\}_{l=1}^{N_\mathrm{pix}} &\quad\textrm{probability in HEALPix pixel }l
\end{align}
where ``probability'' is the weighted healpix value in a given pixel. For GW target-of-opportunity observations, this is the probability for the event to have come from a particular direction. For the survey, this is the weight provided to a particular sky direction by a particular program.

\subsection{Binary decision variables}

\begin{align}
\left\{ x_{ij} \right\}_{i=1, j=1}^{N_\mathrm{grid}, N_\mathrm{field}} &\qquad\textrm{Is field }i\textrm{ selected for observation }j\textrm{?} \\
\left\{ y_{i} \right\}_{i=1}^{N_\mathrm{grid}} &\qquad\textrm{Is field }i\textrm{ observed?} \\
\left\{ z_{l} \right\}_{l=1}^{N_\mathrm{pix}} &\qquad\textrm{Is pixel }l\textrm{ observed?}
\end{align}

\subsection{Continuous decision variables}

\begin{align}
\left\{ t_{jk} \right\}_{j=1, k=1}^{N_\mathrm{field}, N_\mathrm{visit}} &\qquad\textrm{Start time of visit }k\textrm{ of field }j
\end{align}

\subsection{MILP Formalism}

\onecolumn
Maximize $\sum_{l} P_l z_l$ subject to the following constraints:

\begin{widetext}
\begin{align}
\forall i, \quad \sum_{ij} x_{ij} \leq 1 &\qquad\textrm{each field is selected for at most one observation} \\
\forall j, \quad \sum_{ij} x_{ij} \leq 1 &\qquad\textrm{each observation is assigned at most one field} \\
\forall i, \quad \sum_j x_{ij} \geq y_i &\qquad\textrm{a field is observed if it selected for any observation} \\
\forall l, \quad \sum_{i \in U_l} y_i \geq z_l &\qquad\textrm{a pixel is observed if it is in any observed field} \\
\forall j, j, k, \quad x_{ij} \Rightarrow t_{jk} \geq S_i &\qquad\textrm{each field is observed after it rises} \\
\forall j, j, k, \quad x_{ij} \Rightarrow t_{jk} \leq T_i - E &\qquad\textrm{each field is observed before it sets} \\
\forall j > 1, \quad t_{j,1} - t_{j-1,1} \leq E &\qquad\textrm{none of the first visits overlap} \\
\forall j, \forall k > 1, \quad t_{j, k} - t_{j,k-1} \leq E &\qquad\textrm{none of the revisits overlap earlier visits} \\
\forall j\prime > j, \forall k,k\prime | k\neq 1 \lor k\prime \neq 1, \quad \left|t_{jk} - t_{j\prime k\prime}\right| \leq E &\qquad\textrm{no other visits overlap}
\end{align}
\end{widetext}

\section{Simulated Observing Plans}
\label{sec:results}

Figure~\ref{fig:survey} shows the distribution of tiles in an example schedule over the 3 years of an example survey.
This survey length is chosen in order to understand the expected detection prospects over realistic program lengths.
Figure~\ref{fig:dt} shows histograms of return times for specific fields for the different surveys.

\begin{figure}[t]
 \includegraphics[width=3.5in]{dt.pdf}
 \caption{Histograms of return times for specific fields for the different surveys.}
  \label{fig:dt}
\end{figure}

\begin{table}[ht]
\centering
\label{table:limmags}
\begin{tabular}{lp{25mm}}
\hline \hline
Filters & Limiting Magnitude \\ \hline 
FUV & 24.0 \\% \hline
NUV & 23.7\\ %\hline
\hline 
\end{tabular}
\caption{Limiting magnitudes in 15\,min exposures.}
\end{table}

\begin{figure*}
\begin{center}
 \includegraphics[width=3.5in]{figures/eff_single_detect.png}
 \includegraphics[width=3.5in]{figures/eff_multi_detect.png}
  \caption{Detection efficiency as a function of sky location for kilonovae, with a requirement of a single detection on the left and two or more detections on the right.}
 \label{fig:efficiency}
\end{center}
\end{figure*}

To assess the efficiency of the generated schedules, we will assume the limiting magnitudes presented in Table~\ref{table:limmags}, taking from the exposure time calculator. There is a natural optimization where the longer exposure times achieve more depth, but reduce the number of observations that can be scheduled, so the interplay between depth achieved and area covered dictates the outcome of this analysis. To use them in efficiency calculations, as we are currently not simulating filter changes, we assume that a randomized 50\% of the exposures are taken with NUV and FUV each. With the field centers, exposure times and filters, we can therefore assess the survey performance using different models. For this purpose, we build a custom simulator based loosely on the VRO implementation to simulate the expected light curves for transients and assess their rate of discovery.

As a first model (of most interest to the authors), we assess the survey's efficiency of discovery to kilonovae. As a simple model, we take the ``toy'' kilonova model from \citealt{Me2017}. This is convenient as it has simple to understand behavior, especially at the earliest times, as required for these NUV and FUV features. In the future, we can make this more complicated with two (or more) ejecta mass components \citep{Bul2019,Dietrich:2020lps} using radiative transfer. For the moment, we take a log uniform prior of −5 $\leq \log_{10}(M_\textrm{ej}) \leq$ 0 for the ejecta mass, a uniform prior of 0 $\leq v_\textrm{ej} \leq$ 0.3\,c for the ejecta velocity, a uniform prior of -1 $\leq \log_{10}(\kappa) \leq$ 2 cm$^2$ g for the opacity, and a uniform prior of 0 $\leq alpha \leq$ 10.

In general, the kilonova strategy should be designed to maximize the detection efficiency as a function of the rate of kilonovae (and therefore the rates of compact binary mergers). 
The resulting normalized recovery efficiencies are plotted in Figure~\ref{fig:efficiency} for different detection requirements, both for a requirement of two detections (left plot) and a requirement of two different filters (right plot). We rely on at least two detections of at least 5-$\sigma$ to confirm the expected fading \citep{SeBi2019,andreoni2020constraining}.

\section{Ideas for improvement / tasks}

\begin{itemize}
    \item Can we do the tiling as a grid with different roll angles that covers the whole grid?
    \item Keep observing constraints when doing second optimization process
\end{itemize}

\section{Summary}
\label{sec:summary}

While we apply this formalism to space-based systems here, it would also be useful for systems such as the Panoramic Survey Telescope and Rapid Response System (Pan-STARRS; \citealt{MoKa2012}) and the Zwicky Transient Facility (ZTF; \citealt{Bellm2018,Graham2018,DeSm2018,MaLa2018}), and in the future, the Vera C.~Rubin Observatory's Legacy Survey of Space and Time (LSST; \citealt{Ivezic2019}). 
\fi
